Feature Descriptors for Tracking by Detection: a Benchmark

In this paper, we provide an extensive evaluation of the performance of local descriptors for tracking applications. Many different descriptors have been proposed in the literature for a wide range of application in computer vision such as object recognition and 3D reconstruction. More recently, due to fast key-point detectors, local image features can be used in online tracking frameworks. However, while much effort has been spent on evaluating their performance in terms of distinctiveness and robustness to image transformations, very little has been done in the contest of tracking. Our evaluation is performed in terms of distinctiveness, tracking precision and tracking speed. Our results show that binary descriptors like ORB or BRISK have comparable results to SIFT or AKAZE due to a higher number of key-points.

==> additional.tex <==
\section{Additional}

\todo[inline]{Please note this is a collection of tables and images that will not end in the paper. They are good anyway to have a picture of the results}

\begin{figure*}
\centerline{%
	\subfigure{
		\includegraphics[width=0.5\linewidth]{imgs/brisk_correlation.pdf}~
		\includegraphics[width=0.5\linewidth]{imgs/orb_correlation.pdf}~
		}}
\vspace{-2.0mm}
\centerline{%
\subfigure{
		\includegraphics[width=0.5\linewidth]{imgs/akazec_correlation.pdf}~
		\includegraphics[width=0.5\linewidth]{imgs/sift_correlation.pdf}~
		}}
\vspace{-2.0mm}
\addtocounter{subfigure}{-1}
\centerline{%
	\subfigure{	
		\includegraphics[width=0.5\linewidth]{imgs/surf_correlation.pdf}~
		\includegraphics[width=0.5\linewidth]{imgs/cuda_sift_correlation.pdf}~
\label{fig:exp_d}		
}}
\vspace{-2.0mm}
\caption{Correlations matrices between the different evaluated measures of the feature descriptors.}
\vspace{-2mm}
\label{fig:depth_comparison_second}
\end{figure*}

\begin{figure*}[t]
\centerline{% 
		\includegraphics[width=0.98\linewidth]{tables/test.pdf}}
    \vspace{-2mm} 
	\caption{Overall results of the dataset for true positive matching. This is just a preview it won't be in he paper.}
	\label{fig:learnvsno}
\end{figure*}
